Measurement of the helicity asymmetry $\mathbb{E}$ for the $\vec{\gamma}\vec{p} \to p \pi^0$ reaction in the resonance region

The double-spin-polarization observable $\mathbb{E}$ for $\vec{\gamma}\vec{p}\to p\pi^0$ has been measured with the CEBAF Large Acceptance Spectrometer (CLAS) at photon beam energies $E_\gamma$ from 0.367 to $2.173~\mathrm{GeV}$ (corresponding to center-of-mass energies from 1.240 to $2.200~\mathrm{GeV}$) for pion center-of-mass angles, $\cos\theta_{\pi^0}^{c.m.}$, between -0.86 and 0.82. These new CLAS measurements cover a broader energy range and have smaller uncertainties compared to previous CBELSA data and provide an important independent check on systematics. These measurements are compared to predictions as well as new global fits from The George Washington University, Mainz, and Bonn-Gatchina groups. Their inclusion in multipole analyses will refine our understanding of the single-pion production contribution to the Gerasimov-Drell-Hearn sum rule and improve the determination of resonance properties.

==> HelicityAsymmetryPiZero /author_list.tex <==
\newcommand*{\ANL}{Argonne National Laboratory, Argonne, Illinois 60439, United States of America}
\newcommand*{\ANLindex}{1}
\affiliation{\ANL}
\newcommand*{\ASU}{Arizona State University, Tempe, Arizona 85287, United States of America}
\newcommand*{\ASUindex}{2}
\affiliation{\ASU}
\newcommand*{\CSUDH}{California State University, Dominguez Hills, Carson, California 90747, United States of America}
\newcommand*{\CSUDHindex}{3}
\affiliation{\CSUDH}
\newcommand*{\CANISIUS}{Canisius College, Buffalo, New York 14208, United States of America}
\newcommand*{\CANISIUSindex}{4}
\affiliation{\CANISIUS}
\newcommand*{\CMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, United States of America}
\newcommand*{\CMUindex}{5}
\affiliation{\CMU}
\newcommand*{\CUA}{The Catholic University of America, Washington, District of Columbia 20064, United States of America}
\newcommand*{\CUAindex}{6}
\affiliation{\CUA}
\newcommand*{\SACLAY}{IRFU, CEA, Universit\`{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\newcommand*{\SACLAYindex}{7}
\affiliation{\SACLAY}
\newcommand*{\CNU}{Christopher Newport University, Newport News, Virginia 23606, United States of America}
\newcommand*{\CNUindex}{8}
\affiliation{\CNU}
\newcommand*{\UCONN}{University of Connecticut, Storrs, Connecticut 06269, United States of America}
\newcommand*{\UCONNindex}{9}
\affiliation{\UCONN}
\newcommand*{\DUQUESNE}{Duquesne University, Pittsburgh, Pennsylvania 15282, United States of America }
\newcommand*{\DUQUESNEindex}{10}
\affiliation{\DUQUESNE}
\newcommand*{\FU}{Fairfield University, Fairfield, Connecticut 06824, United States of America}
\newcommand*{\FUindex}{11}
\affiliation{\FU}
\newcommand*{\FERRARAU}{Universit\`a di Ferrara, 44121 Ferrara, Italy}
\newcommand*{\FERRARAUindex}{12}
\affiliation{\FERRARAU}
\newcommand*{\FIU}{Florida International University, Miami, Florida 33199, United States of America}
\newcommand*{\FIUindex}{13}
\affiliation{\FIU}
\newcommand*{\FSU}{Florida State University, Tallahassee, Florida 32306, United States of America}
\newcommand*{\FSUindex}{14}
\affiliation{\FSU}
\newcommand*{\GWUI}{The George Washington University, Washington, District of Columbia 20052, United States of America}
\newcommand*{\GWUIindex}{15}
\affiliation{\GWUI}
\newcommand*{\GSIFFN}{GSI Helmholtzzentrum fur Schwerionenforschung GmbH, D-64291 Darmstadt, Germany}
\newcommand*{\GSIFFNindex}{16}
\affiliation{\GSIFFN}
\newcommand*{\INFNFE}{INFN, Sezione di Ferrara, 44100 Ferrara, Italy}
\newcommand*{\INFNFEindex}{17}
\affiliation{\INFNFE}
\newcommand*{\INFNGE}{INFN, Sezione di Genova, 16146 Genova, Italy}
\newcommand*{\INFNGEindex}{18}
\affiliation{\INFNGE}
\newcommand*{\INFNRO}{INFN, Sezione di Roma Tor Vergata, 00133 Rome, Italy}
\newcommand*{\INFNROindex}{19}
\affiliation{\INFNRO}
\newcommand*{\INFNTUR}{INFN, Sezione di Torino, 10125 Torino, Italy}
\newcommand*{\INFNTURindex}{20}
\affiliation{\INFNTUR}
\newcommand*{\INFNPAV}{INFN, Sezione di Pavia, 27100 Pavia, Italy}
\newcommand*{\INFNPAVindex}{21}
\affiliation{\INFNPAV}
\newcommand*{\IFKMA}{Institut f\"ur Kernphysik, Johannes Gutenberg University of Mainz, D-55099 Mainz, Germany}
\newcommand*{\IFKMAindex}{22}
\affiliation{\IFKMA}
\newcommand*{\KNU}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand*{\KNUindex}{23}
\affiliation{\KNU}
\newcommand*{\LAMAR}{Lamar University, Beaumont, Texas 77710, United States of America}
\newcommand*{\LAMARindex}{24}
\affiliation{\LAMAR}
\newcommand*{\MIT}{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139, United States of America}
\newcommand*{\MITindex}{25}
\affiliation{\MIT}
\newcommand*{\MISS}{Mississippi State University, Mississippi State, Mississippi 39762, United States of America}
\newcommand*{\MISSindex}{26}
\affiliation{\MISS}
\newcommand*{\ITEP}{National Research Centre Kurchatov Institute - ITEP, Moscow, 117259, Russia}
\newcommand*{\ITEPindex}{27}
\affiliation{\ITEP}
\newcommand*{\NMSU}{New Mexico State University, Las Cruces, New Mexico 88003, United States of America}
\newcommand*{\NMSUindex}{28}
\affiliation{\NMSU}
\newcommand*{\NSU}{Norfolk State University, Norfolk, Virginia 23504, United States of America}
\newcommand*{\NSUindex}{29}
\affiliation{\NSU}
\newcommand*{\NRC}{NRC Kurchatov Institute, PNPI, Gatchina 188300, Russia}
\newcommand*{\NRCindex}{30}
\affiliation{\NRC}
\newcommand*{\OHIOU}{Ohio University, Athens, Ohio 45701, United States of America}
\newcommand*{\OHIOUindex}{31}
\affiliation{\OHIOU}
\newcommand*{\ODU}{Old Dominion University, Norfolk, Virginia 23529, United States of America}
\newcommand*{\ODUindex}{32}
\affiliation{\ODU}
\newcommand*{\JLUGiessen}{II Physikalisches Institut, Justus Liebig University Giessen, 35392 Giessen, Germany}
\newcommand*{\JLUGiessenindex}{33}
\affiliation{\JLUGiessen}
\newcommand*{\MSU}{Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, 119234 Moscow, Russia}
\newcommand*{\MSUindex}{34}
\affiliation{\MSU}
\newcommand*{\TEMPLE}{Temple University,  Philadelphia, Pennsylvania 19122, United States of America }
\newcommand*{\TEMPLEindex}{35}
\affiliation{\TEMPLE}
\newcommand*{\JLAB}{Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606, United States of America}
\newcommand*{\JLABindex}{36}
\affiliation{\JLAB}

\newcommand*{\ORSAY}{Universit\`{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand*{\ORSAYindex}{37}
\affiliation{\ORSAY}
\newcommand*{\UNH}{University of New Hampshire, Durham, New Hampshire 03824, United States of America}
\newcommand*{\UNHindex}{38}
\affiliation{\UNH}
\newcommand*{\URICH}{University of Richmond, Richmond, Virginia 23173, United States of America}
\newcommand*{\URICHindex}{39}
\affiliation{\URICH}
\newcommand*{\ROMAII}{Universit\`a di Roma Tor Vergata, 00133 Rome Italy}
\newcommand*{\ROMAIIindex}{40}
\affiliation{\ROMAII}
\newcommand*{\SCAROLINA}{University of South Carolina, Columbia, South Carolina 29208, United States of America}
\newcommand*{\SCAROLINAindex}{41}
\affiliation{\SCAROLINA}
\newcommand*{\UTFSM}{Universidad T\`{e}cnica Federico Santa Mar\'{i}a, Casilla 110-V Valpara\`{i}so, Chile}
\newcommand*{\UTFSMindex}{42}
\affiliation{\UTFSM}
\newcommand*{\BRESCIA}{Universit\`{a} degli Studi di Brescia, 25123 Brescia, Italy}
\newcommand*{\BRESCIAindex}{43}
\affiliation{\BRESCIA}
\newcommand*{\UCR}{University of California Riverside, Riverside, California 92521, United States of America}
\newcommand*{\UCRindex}{44}
\affiliation{\UCR}
\newcommand*{\GLASGOW}{University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\newcommand*{\GLASGOWindex}{45}
\affiliation{\GLASGOW}
\newcommand*{\YORK}{University of York, York YO10 5DD, United Kingdom}
\newcommand*{\YORKindex}{46}
\affiliation{\YORK}
\newcommand*{\VT}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, United States of America}
\newcommand*{\VTindex}{47}
\affiliation{\VT}
\newcommand*{\VIRGINIA}{University of Virginia, Charlottesville, Virginia 22901, United States of America}
\newcommand*{\VIRGINIAindex}{48}
\affiliation{\VIRGINIA}
\newcommand*{\WM}{College of William and Mary, Williamsburg, Virginia 23187, United States of America}
\newcommand*{\WMindex}{49}
\affiliation{\WM}
\newcommand*{\YEREVAN}{Yerevan Physics Institute, 375036 Yerevan, Armenia}
\newcommand*{\YEREVANindex}{50}
\affiliation{\YEREVAN}
\newcommand*{\NOWJLAB}{Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606, United States of America}
\newcommand*{\NOWVIRGINIA}{University of Virginia, Charlottesville, Virginia 22901, United States of America}
\newcommand*{\NOWMERYLAND}{Montgomery College, Germantown, Maryland 20876, United States of America}
 %%%%%%%%%%%%%%% END OF Latex Macros for institute addresses  %%%%%%%%%%%%%%%%%%%%%%%%% 


\author{\mbox{C.~W.~Kim}}
\affiliation{\GWUI}

\author{\mbox{N.~Zachariou}}
\altaffiliation{Corresponding author: \texttt{nick.zachariou@york.ac.uk}}
\affiliation{\YORK}

\author{\mbox{M.~Bashkanov}}
\affiliation{\YORK}

\author{\mbox{W.~J.~Briscoe}}
\affiliation{\GWUI}

\author{\mbox{S.~Fegan}}
 \affiliation{\YORK}

\author{\mbox{V.~L.~Kashevarov}}
\affiliation{\IFKMA}

\author{\mbox{K.~Nikonov}}
\affiliation{\NRC}

\author{\mbox{A.~Sarantsev}}
\affiliation{\NRC}

\author{\mbox{A.~Schmidt}}
\affiliation{\GWUI}

\author{\mbox{I.~I.~Strakovsky}}
\affiliation{\GWUI}

\author{\mbox{D.~P.~Watts}}
\affiliation{\YORK}

\author{\mbox{R.~L.~Workman}}
\affiliation{\GWUI}

\author {P.~Achenbach} 
\affiliation{\JLAB}
\author {Z.~Akbar} 
\affiliation{\VIRGINIA}
\author {M.~J.~Amaryan} 
\affiliation{\ODU}
\author{\mbox{G.~Angelini}}
\affiliation{\GWUI}
\author {W.~R.~Armstrong} 
\affiliation{\ANL}
\author {H.~Atac} 
\affiliation{\TEMPLE}
\author {L.~Baashen} 
\affiliation{\FIU}
\author {N.~A.~Baltzell} 
\affiliation{\JLAB}
\affiliation{\SCAROLINA}
\author {L.~Barion} 
\affiliation{\INFNFE}
\author {M.~Battaglieri} 
\affiliation{\INFNGE}
\author {I.~Bedlinskiy} 
\affiliation{\ITEP}
\author {B.~Benkel} 
\affiliation{\UTFSM}
\author {F.~Benmokhtar} 
\affiliation{\DUQUESNE}
\author{\mbox{N.~Benmouna}}
\altaffiliation[Current address:]{\NOWMERYLAND}
% \altaffiliation{Current address:  Montgomery College, Germantown, Maryland 20876, United States of America}
\affiliation{\GWUI}
\author {A.~Bianconi} 
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {A.~S.~Biselli} 
\affiliation{\FU}
\author {W.~A.~Booth} 
\affiliation{\YORK}
\author {F.~Boss\`u} 
\affiliation{\SACLAY}
\author {S.~Boiarinov} 
\affiliation{\JLAB}
\author {K.~T.~Brinkmann} 
\affiliation{\JLUGiessen}
\author{\mbox{J.~Brock}}
\affiliation{\JLAB}
\author {D.~Bulumulla} 
\affiliation{\ODU}
\author {V.~D.~Burkert} 
\affiliation{\JLAB}
\author {T.~Cao} 
\affiliation{\JLAB}
\author{\mbox{C.~Carlin}}
\affiliation{\JLAB}
\author {D.~S.~Carman} 
\affiliation{\JLAB}
\author {J.~C.~Carvajal} 
\affiliation{\FIU}
\author {P.~Chatagnon} 
\affiliation{\JLAB}
\author {V.~Chesnokov} 
\affiliation{\MSU}
\author {T.~Chetry} 
\affiliation{\FIU}
\author {G.~Ciullo} 
\affiliation{\INFNFE}
\affiliation{\FERRARAU}
\author {G.~Clash} 
\affiliation{\YORK}
\author {P.~L.~Cole} 
\affiliation{\LAMAR}
\author {M.~Contalbrigo} 
\affiliation{\INFNFE}
\author{\mbox{O.~Cortes~Becerra}}
\affiliation{\GWUI}
\author {G.~Costantini} 
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {V.~Crede} 
\affiliation{\FSU}
\author {A.~D'Angelo} 
\affiliation{\INFNRO}
\affiliation{\ROMAII}
\author {N.~Dashyan} 
\affiliation{\YEREVAN}
\author {R.~De~Vita} 
\affiliation{\INFNGE}
\author {M.~Defurne} 
\affiliation{\SACLAY}
\author {A.~Deur} 
\affiliation{\JLAB}
\author {S.~Diehl} 
\affiliation{\JLUGiessen}
\affiliation{\UCONN}
\author {C.~Djalali} 
\affiliation{\OHIOU}
\affiliation{\SCAROLINA}
\author {M.~Dugger} 
\affiliation{\ASU}
\author {R.~Dupre} 
\affiliation{\ORSAY}
\author {H.~Egiyan} 
\affiliation{\JLAB}
\affiliation{\UNH}
\author {A.~El~Alaoui} 
\affiliation{\UTFSM}
\author {L.~El~Fassi} 
\affiliation{\MISS}
\affiliation{\ANL}
\author {L.~Elouadrhiri} 
\affiliation{\JLAB}
\author {P.~Eugenio} 
\affiliation{\FSU}
\author {A.~Filippi} 
\affiliation{\INFNTUR}
\author {C.~Fogler} 
\affiliation{\ODU}
\author {G.~Gavalian} 
\affiliation{\JLAB}
\affiliation{\ODU}
\author {G.~P.~Gilfoyle} 
\affiliation{\URICH}
\author {A.~A.~Golubenko} 
\affiliation{\MSU}
\author{G.~Gosta}
\affiliation{\INFNPAV}
\author {R.~W.~Gothe} 
\affiliation{\SCAROLINA}
\author {K.~A.~Griffioen} 
\affiliation{\WM}
\author {K.~Hafidi} 
\affiliation{\ANL}
\author {H.~Hakobyan} 
\affiliation{\UTFSM}
\affiliation{\YEREVAN}
\author {M.~Hattawy} 
\affiliation{\ODU}
\author {F.~Hauenstein} 
\affiliation{\JLAB}
\author {T.~B.~Hayward} 
\affiliation{\UCONN}
\author {D.~Heddle} 
\affiliation{\CNU}
\affiliation{\JLAB}
\author {A.~Hobart} 
\affiliation{\ORSAY}
\author {M.~Holtrop} 
\affiliation{\UNH}
\author {Y.~Ilieva} 
\affiliation{\SCAROLINA}
\affiliation{\GWUI}
\author{\mbox{I.~Illari}}
\affiliation{\GWUI}
\author {D.~G.~Ireland} 
\affiliation{\GLASGOW}
\author {E.~L.~Isupov} 
\affiliation{\MSU}
\author{\mbox{H.~Iwamoto}}
\affiliation{\GWUI}
\author {D.~Jenkins} 
\affiliation{\VT}
\author {H.~S.~Jo} 
\affiliation{\KNU}
\author {R.~Johnston} 
\affiliation{\MIT}
\author {K.~Joo} 
\affiliation{\UCONN}
\author {S.~Joosten} 
\affiliation{\ANL}
\author {T.~Kageya} 
\affiliation{\JLAB}
\author{\mbox{C.~D.~Keith}}
\affiliation{\JLAB}
\author {D.~Keller} 
\affiliation{\VIRGINIA}
\affiliation{\OHIOU}
\author {A.~Khanal} 
\affiliation{\FIU}
\author {A.~Kim} 
\affiliation{\UCONN}
\author {W.~Kim} 
\affiliation{\KNU}
\author {F.~J.~Klein} 
\affiliation{\CUA}
\author {V.~Klimenko} 
\affiliation{\UCONN}
\author {A.~Kripko} 
\affiliation{\JLUGiessen}
\author {V.~Kubarovsky} 
\affiliation{\JLAB}
\author {L.~Lanza} 
\affiliation{\INFNRO}
\affiliation{\ROMAII}
\author {M.~Leali} 
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {S.~Lee} 
\affiliation{\ANL}
\author {X.~Li} 
\affiliation{\MIT}
\author {K.~Livingston} 
\affiliation{\GLASGOW}
\author {I.~J.~D.~MacGregor} 
\affiliation{\GLASGOW}
\author {D.~Marchand} 
\affiliation{\ORSAY}
\author {V.~Mascagna} 
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {B.~McKinnon} 
\affiliation{\GLASGOW}
\author {S.~Migliorati} 
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {R.~G.~Milner} 
\affiliation{\MIT}
\author {T.~Mineeva} 
\affiliation{\UTFSM}
\author {V.~Mokeev} 
\affiliation{\JLAB}
\affiliation{\MSU}
\author {C.~Munoz~Camacho} 
\affiliation{\ORSAY}
\author {P.~Nadel-Turonski} 
\affiliation{\JLAB}
\affiliation{\CUA}
\author {K.~Neupane} 
\affiliation{\SCAROLINA}
\author {S.~Niccolai} 
\affiliation{\ORSAY}
\author {M.~Osipenko} 
\affiliation{\INFNGE}
\author {A.~I.~Ostrovidov} 
\affiliation{\FSU}
\author {P.~Pandey} 
\affiliation{\ODU}
\author {M.~Paolone} 
\affiliation{\NMSU}
\author {L.~L.~Pappalardo} 
\affiliation{\INFNFE}
\affiliation{\FERRARAU}
\author {R.~Paremuzyan} 
\affiliation{\JLAB}
\author {E.~Pasyuk} 
\affiliation{\JLAB}
\author {S.~J.~Paul} 
\affiliation{\UCR}
\author {N.~Pilleux} 
\affiliation{\ORSAY}
\author {M.~Pokhrel} 
\affiliation{\ODU}
\author {J.~Poudel} 
\altaffiliation[Current address:]{\NOWJLAB}
\affiliation{\ODU}
\author {J.~W.~Price} 
\affiliation{\CSUDH}
\author {Y.~Prok} 
\affiliation{\ODU}
\affiliation{\VIRGINIA}
\author {A.~Radic} 
\affiliation{\UTFSM}
\author {N.~Ramasubramanian} 
\affiliation{\SACLAY}
\author{\mbox{S.~Ratliff}}
\affiliation{\GWUI}
\author {T.~Reed} 
\affiliation{\FIU}
\author {J.~Richards} 
\affiliation{\UCONN}
\author {M.~Ripani} 
\affiliation{\INFNGE}
\author {B.~G.~Ritchie} 
\affiliation{\ASU}
\author {J.~Ritman} 
\affiliation{\GSIFFN}
\author {G.~Rosner} 
\affiliation{\GLASGOW}
\author {C.~Salgado} 
\affiliation{\NSU}
\author {S.~Schadmand} 
\affiliation{\GSIFFN}
\author{\mbox{D.~Schott}}
\altaffiliation{Current address: University of Nebraska, 
        Omaha, Nebraska 68198, United States of America}
\affiliation{\GWUI}
\author {R.~A.~Schumacher} 
\affiliation{\CMU}
\author {M.~B.~C~Scott} 
\affiliation{\ANL}
\author{\mbox{M.~L.~Seely}}
\affiliation{\JLAB}
\author{\mbox{E.~M.~Seroka}}
\affiliation{\GWUI}
\author {E.~V.~Shirokov} 
\affiliation{\MSU}
\author {U.~Shrestha} 
\affiliation{\UCONN}
\author {D.~Sokhan} 
\affiliation{\SACLAY}
\affiliation{\GLASGOW}
\author {N.~Sparveris} 
\affiliation{\TEMPLE}
\author {M.~Spreafico} 
\affiliation{\INFNGE}
\author {S.~Strauch} 
\affiliation{\SCAROLINA}
\author {J.~Tan} 
\affiliation{\KNU}
\author {R.~Tyson} 
\affiliation{\GLASGOW}
\author {M.~Ungaro} 
\affiliation{\JLAB}
\affiliation{\UCONN}
\author {S.~Vallarino} 
\affiliation{\INFNFE}
\author {L.~Venturelli} 
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {H.~Voskanyan} 
\affiliation{\YEREVAN}
\author{E.~Voutier}
\affiliation{\ORSAY}
\author {X.~Wei} 
\affiliation{\JLAB}
\author {R.~Williams} 
\affiliation{\YORK}
\author {R.~Wishart} 
\affiliation{\GLASGOW}
\author {M.~H.~Wood} 
\affiliation{\CANISIUS}
\affiliation{\SCAROLINA}
\author{M.~Yurov}
\affiliation{\MISS}
\author {J.~Zhang} 
\altaffiliation[Current address:]{\NOWVIRGINIA}
\affiliation{\ODU}
\author {M.~Zurek} 
\affiliation{\ANL}

\collaboration{The CLAS Collaboration}
\noaffiliation


==> HelicityAsymmetryPiZero /references.tex <==
\begin{thebibliography}{99}
\bibitem{CLAS:2017kua}
    D.~Ho \textit{et al.} [CLAS Collaboration],
    ``Beam-target helicity asymmetry for $\stackrel{\ensuremath{\rightarrow}}{\ensuremath{\gamma}}\stackrel{\ensuremath{\rightarrow}}{n}\ensuremath{\rightarrow}{\ensuremath{\pi}}^{\ensuremath{-}}p$ in the ${N}^{*}$ resonance region,''
    Phys.\ Rev.\ Lett.\ \textbf{118}, 242002 (2017).
\bibitem{Anisovich:2016vzt}
    A.~V.~Anisovich, R.~Beck, M.~D\"oring, M.~Gottschall, J.~Hartmann, V.~Kashevarov, E.~Klempt, U.~G.~Mei\ss{}ner, V.~Nikonov, M.~Ostrick \textit{et al.}
    ``The impact of new polarization data from Bonn, Mainz and Jefferson Laboratory on $\gamma p \rightarrow \pi N$ multipoles,''
    Eur.\ Phys.\ J.\ A\ \textbf{52}, 284 (2016).
\bibitem{ParticleDataGroup:2022pth}
    R.~L.~Workman \textit{et al.} [Particle Data Group],
    Prog.\ Theor.\ Exp.\ Phys.\ \textbf{2022}, 083C01 (2022).
\bibitem{Ronchen:2015vfa}
    D.~R\"onchen, M.~D\"oring, H.~Haberzettl, J.~Haidenbauer, U.~G.~Mei\ss{}ner, and K.~Nakayama,
    ``Eta photoproduction in a combined analysis of pion- and photon-induced reactions,''
    Eur.\ Phys.\ J.\ A\ \textbf{51}, 70 (2015).
\bibitem{CBELSATAPS:2014wvh}
     The Bonn-Gatchina analyses are available through the Bonn website: 
     http://pwa.hiskp.uni-bonn.de/; see also
    E.~Gutz \textit{et al.} [CBELSA/TAPS Collaboration],
    ``High statistics study of the reaction $\gamma p\to p\pi^0\eta$,''
    Eur.\ Phys.\ J.\ A\ \textbf{50}, 74 (2014).
\bibitem{Kamano:2013iva}
    H.~Kamano, S.~X.~Nakamura, T.~S.~H.~Lee, and T.~Sato,
    ``Nucleon resonances within a dynamical coupled-channels model of $\pi N$ and $\gamma N$ reactions,''
    Phys.\ Rev.\ C\ \textbf{88}, 035209 (2013).
\bibitem{Ireland:2019uwn}
    D.~G.~Ireland, E.~Pasyuk, and I.~Strakovsky,
    ``Photoproduction reactions and non-strange baryon spectroscopy,''
    Prog.\ Part.\ Nucl.\ Phys.\ \textbf{111}, 103752 (2020).
\bibitem{Zachariou:G}
    N.~Zachariou \textit{et al.} [CLAS Collaboration],
    ``Double polarisation observable $\mathbb{G}$ for single pion photoproduction from the proton,''
    Phys.\ Lett.\ B\ \textbf{817}, 136304 (2021).
\bibitem{CLAS:2015ykk}
    S.~Strauch \textit{et al.} [CLAS Collaboration],
    ``First measurement of the polarization observable $\mathbb{E}$ in the $\vec{p}$($\vec{\gamma},\pi^+$)$n$ reaction up to 2.25~GeV",
    Phys.\ Lett.\ B\ \textbf{750}, 53 (2015).
\bibitem{CLAS:2018gxz}
    D.~Ho \textit{et al.} [CLAS Collaboration],
    ``Beam-target helicity asymmetry $\mathbb{E}$ in ${K}^{0}\mathrm{\ensuremath{\Lambda}}$ and ${K}^{0}{\mathrm{\ensuremath{\Sigma}}}^{0}$ photoproduction on the neutron,''
    Phys.\ Rev.\ C\ \textbf{98}, 045205 (2018).
\bibitem{CLAS:2020spy}
    N.~Zachariou \textit{et al.} [CLAS Collaboration],
    ``Beam-target helicity asymmetry $\mathbb{E}$ in $K^+\Sigma^-$ photoproduction on the neutron,''
    Phys.\ Lett.\ B\ \textbf{808}, 135662 (2020).
\bibitem{Keith:2012ad}
    C.~D.~Keith, J.~Brock, C.~Carlin, S.~A.~Comer, D.~Kashy, J.~McAndrew, D.~G.~Meekins, E.~Pasyuk, J.~J.~Pierce, and M.~L.~Seely,
    ``The Jefferson Lab Frozen Spin Target,''
    Nucl.\ Instrum.\ Meth.\ A\ \textbf{684}, 27 (2012).
\bibitem{Strakovsky:2022tvu}
    I.~Strakovsky, S.~\v{S}irca, W.~J.~Briscoe, A.~Deur, A.~Schmidt, and R.~L.~Workman,
    ``Single-pion contribution to the Gerasimov-Drell-Hearn sum rule and related integrals,''
    Phys.\ Rev.\ C\ \textbf{105}, 045202 (2022).
\bibitem{CBELSATAPS:2013btn}
    M.~Gottschall \textit{et al.} [CBELSA/TAPS Collaboration],
    ``First measurement of the helicity asymmetry for $\gamma p\rightarrow p\pi^0$ in the resonance region,''
    Phys.\ Rev.\ Lett.\ \textbf{112}, 012003 (2014).
\bibitem{Walker:1968xu}
     R.~Walker, 
     ``Phenomenological analysis of single pion production,'' 
     Phys.\ Rev.\ \textbf{182}, 1729 (1969).
\bibitem{Barker:1975bp}
     I.~S.~Barker, A.~Donnachie, and J.~K.~Storrow,
     ``Complete experiments in pseudoscalar photoproduction,''
     Nucl.\ Phys.\ B\ \textbf{95}, 347 (1975).
\bibitem{Workman:1991xs}
     R.~L.~Workman and R.~A.~Arndt,
     ``Saturation of the Drell-Hearn-Gerasimov sum rule revisited,''
     Phys.\ Rev.\ D\ \textbf{45}, 1789 (1992).
\bibitem{Chiang:1996em}
    W.-T.~Chiang and F.~Tabakin, 
    ``Completeness rules for spin observables in pseudoscalar meson photoproduction,''
    Phys.\ Rev. \ C\ \textbf{55}, 2054 (1997).
\bibitem{Nakayama:2019cys}
    K.~Nakayama, 
    ``On the spin-observables in pseudoscalar meson photoproduction,''
    J.\ Phys.\ G\ \textbf{46}, 105108 (2019).
\bibitem{Svarc:2017yuo}
    A.~\v{S}varc, Y.~Wunderlich, H.~Osmanovi\'c, M.~Had\v{z}imehmedovi\'c, R.~Omerovi\'c, J.~Stahov, V.~Kashevarov, K.~Nikonov, M.~Ostrick, L.~Tiator \textit{et al.}
    ``Connection between angle-dependent phase ambiguities and the uniqueness of the partial-wave decomposition,''
    Phys.\ Rev.\ C\ \textbf{97}, 054611 (2018).
\bibitem{Wunderlich:2017dby}
    Y.~Wunderlich, A.~\v{S}varc, R.~L.~Workman, L.~Tiator, and R.~Beck,
    ``Toward an understanding of discrete ambiguities in truncated partial-wave analyses,''
    Phys.\ Rev.\ C\ \textbf{96}, 065202 (2017).
\bibitem{Workman:2016irf}
    R.~L.~Workman, L.~Tiator, Y.~Wunderlich, M.~D\"oring, and H.~Haberzettl, 
    ``Amplitude reconstruction from complete photoproduction experiments and truncated partial-wave expansions,''
    Phys.\ Rev.\ C\ \textbf{95}, 015206 (2017).
\bibitem{9a}
    ``Pion photoproduction from a polarized target,'' Spokespersons: N.~Benmouna, W.~J.~Briscoe, 
    G.~V.~O'Rielly, I.~I.~Strakovsky, and S.~Strauch [CLAS Collaborations], JLab Proposal E--03--105, Newport News, VA, USA, 2003.
\bibitem{Leemann:2001dg}
    C.~W.~Leemann, D.~R.~Douglas, and G.~A.~Krafft,
    ``The Continuous Electron Beam Accelerator Facility: CEBAF at the Jefferson Laboratory,''
    Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ \textbf{51}, 413 (2001).
\bibitem{CLAS:2003umf}
    B.~A.~Mecking \textit{et al.},
    ``The CEBAF Large Acceptance Spectrometer (CLAS),''
    Nucl.\ Instrum.\ Meth.\ A\ \textbf{503}, 513 (2003).
\bibitem{Mestayer:2000we}
    M.~D.~Mestayer, D.~S.~Carman, B.~Asavapibhop, F.~J.~Barbosa, P.~Bonneau, S.~B.~Christo, G.~E.~Dodge, T.~Dooling, W.~S.~Duncan, S.~A.~Dytman \textit{et al.}
    ``The CLAS drift chamber system,''
    Nucl.\ Instrum.\ Meth.\ A\ \textbf{449}, 81 (2000).
\bibitem{Smith:1999ii}
    E.~S.~Smith, T.~Carstens, J.~Distelbrink, M.~Eckhause, H.~Egiyan, L.~Elouadrhiri, J.~Ficenec, M.~Guidal, A.~D.~Hancock, F.~W.~Hersman \textit{et al.}
    ``The time-of-flight system for CLAS,''
    Nucl.\ Instrum.\ Meth.\ A\ \textbf{432}, 265 (1999).
\bibitem{Amarian:2001zs}
    M.~Amarian, G.~Asrian, K.~Beard, W.~Brooks, V.~Burkert, T.~Carstens, A.~Coleman, R.~Demirchian, Y.~Efremenko, H.~Egiian \textit{et al.}
    ``The CLAS forward electromagnetic calorimeter,''
    Nucl.\ Instrum.\ Meth.\ A \textbf{460}, 239 (2001).
\bibitem{Sharabian:2005kq}
    Y.~G.~Sharabian, M.~Battaglieri, V.~D.~Burkert, R.~De Vita, L.~Elouadrhiri, L.~Guo, D.~Kashy, V.~Kubarovsky, G.~S.~Mutchler, M.~Ostrick \textit{et al.}
    ``A new highly segmented start counter for the CLAS detector,''
    Nucl.\ Instrum.\ Meth.\ A\ \textbf{556}, 246 (2006).
\bibitem{Sober:2000we}
    D.~I.~Sober, H.~Crannell, A.~Longhi, S.~K.~Matthews, J.~T.~O'Brien, B.~L.~Berman, W.~J.~Briscoe, P.~L.~Cole, J.~P.~Connelly, W.~R.~Dodge \textit{et al.}
    ``The bremsstrahlung tagged photon beam in Hall~B at JLab,''
    Nucl.\ Instrum.\ Meth.\ A\ \textbf{440}, 263 (2000).
\bibitem{Olsen:1959zz}
    H.~Olsen and L.~C.~Maximon,
    ``Photon and electron polarization in high-energy bremsstrahlung and pair production with screening,''
    Phys.\ Rev.\ \textbf{114}, 887 (1959).
\bibitem{Moller}
    C.~K.~Sinclair, 
    ``Electron beam polarimetry,'' 
    Thomas Jefferson National Accelerator Facility (U.~S.) (1998).
\bibitem{Goertz:2002vv}
    S.~Goertz, W.~Meyer, and G.~Reicherz,
    ``Polarized H, D, and He-3 targets for particle physics experiments,''
    Prog.\ Part.\ Nucl.\ Phys.\ \textbf{49}, 403 (2002)
    [erratum: Prog.\ Part.\ Nucl.\ Phys.\ \textbf{51}, 309 (2003)].
%--------------------------------------------------------------------
\bibitem{CLAS:2015pjm}
    I.~Senderovich \textit{et al.} [CLAS Collaboration],
    ``First measurement of the helicity asymmetry $\mathbb{E}$ in $\eta$ photoproduction on the proton,''
    Phys.\ Lett.\ B\ \textbf{755}, 64 (2016).
\bibitem{CLAS:2017yjv}
    Z.~Akbar \textit{et al.} [CLAS Collaboration],
    ``Measurement of the helicity asymmetry $\mathbb{E}$ in $\omega\to\pi^+\pi^-\pi^0$ photoproduction,''
    Phys.\ Rev.\ C\ \textbf{96}, 065209 (2017).
\bibitem{CLAS:2017jrx}
    P.~Roy \textit{et al.} [CLAS Collaboration],
    ``Measurement of the beam asymmetry $\Sigma$ and the target asymmetry $\mathbb{T}$ in the photoproduction of $\omega$ mesons off the proton using CLAS at Jefferson Laboratory,''
    Phys.\ Rev.\ C\ \textbf{97}, 055202 (2018).
\bibitem{CLAS:2018mmb}
    P.~Roy \textit{et al.} [CLAS Collaboration],
    ``First measurements of the double-polarization observables $\mathbb{F}$, $\mathbb{P}$, and $\mathbb{H}$ in \ensuremath{\omega} photoproduction off transversely polarized protons in the $N^\ast$ resonance region,''
    Phys.\ Rev.\ Lett.\ \textbf{122}, 162301 (2019).
\bibitem{CLAS:2021udy}
    N.~Zachariou \textit{et al.} [CLAS Collaboration],
    ``Double polarisation observable $\mathbb G$ for single pion photoproduction from the proton,''
    Phys.\ Lett.\ B\ \textbf{817}, 136304 (2021).
%--------------------------------------------------------------------
\bibitem{CLAS:2013pcs}
    M.~Dugger \textit{et al.} [CLAS Collaboration],
    ``Beam asymmetry $\Sigma$ for $\pi^+$ and $\pi^0$ photoproduction on the proton for photon energies from 1.102 to $1.862~\mathrm{GeV}$,''
    Phys.\ Rev.\ C\ \textbf{88}, 065203 (2013).
\bibitem{Briscoe:2022wj}
    W.~J.~Briscoe, A.~Schmidt, I.~Strakovsky, R.~L.~Workman, and Alfred \v{S}varc,
    ``Extended SAID partial-wave analysis of pion photoproduction,''
    in progress.
\bibitem{Kashevarov:2017vyl}
    V.~L.~Kashevarov, M.~Ostrick, and L.~Tiator,
    ``Regge phenomenology in $\pi^0$ and $\eta$ photoproduction,''
    Phys.\ Rev.\ C\ \textbf{96}, 035207 (2017).
\bibitem{CBELSATAPS:2022uad}
    T.~Seifen \textit{et al.} [CBELSA/TAPS Collaboration],
    ``Polarization observables in double neutral pion photoproduction,''
    [arXiv:2207.01981 [nucl-ex]].
\bibitem{Arndt2006bf}
    R.~A.~Arndt, W.~J.~Briscoe, I.~I.~Strakovsky, and R.~L.~Workman,
    ``Extended partial-wave analysis of $\pi N$ scattering data,''
    Phys.\ Rev.\ C\ \textbf{74}, 045205 (2006).
\bibitem{Paris:2010tz}
    M.~W.~Paris and R.~L.~Workman,
    `Toward a unified description of hadro- and photoproduction: $S$-wave $\pi^-$ and $\eta^-$photoproduction amplitudes,''
    Phys.\ Rev.\ C\ \textbf{82}, 035202 (2010).
\bibitem{Arndt:1985vj}
    R.~A.~Arndt, J.~M.~Ford, and L.~D.~Roper,
    ``Pion - nucleon partial wave analysis to 1100-MeV,''
    Phys.\ Rev.\ D\ \textbf{32}, 1085 (1985).
\bibitem{Workman:2012hx}
    R.~L.~Workman, R.~A.~Arndt, W.~J.~Briscoe, M.~W.~Paris, and I.~I.~Strakovsky,
    ``Parameterization dependence of $T$ matrix poles and eigenphases from a fit to $\pi N$ elastic scattering data,''
    Phys.\ Rev.\ C\ \textbf{86}, 035202 (2012).
\bibitem{Drechsel:2007if}
    D.~Drechsel, S.~S.~Kamalov, and L.~Tiator,
    ``Unitary Isobar Model - MAID2007,''
    Eur.\ Phys.\ J.\ A\ \textbf{34}, 69 (2007).
\bibitem{Guidal:1997hy}
    M.~Guidal, J.~M.~Laget, and M.~Vanderhaeghen,
    ``Pion and kaon photoproduction at high-energies: Forward and intermediate angles,''
    Nucl.\ Phys.\ A\ \textbf{627}, 645 (1997).
\bibitem{Laget:2019tou}
    J.~M.~Laget,
    ``Exclusive meson photo- and electro-production, a window on the structure of hadronic matter,''
    Prog.\ Part.\ Nucl.\ Phys.\ \textbf{111}, 103737 (2020).
\bibitem{Anisovich:2011zz}
    A.~V.~Anisovich, V.~A.~Nikonov, A.~V.~Sarantsev, V.~V.~Anisovich, M.~A.~Matveev, T.~O.~Vulfs, K.~V.~Nikonov, and J.~Nyiri,
    ``Analysis of the meson-meson data in the framework of the dispersion $D$-matrix method,''
    Phys.\ Rev.\ D\ \textbf{84}, 076001 (2011).
\bibitem{Kashevarov:2022}
    V.~L.~Kashevarov and L.~Tiator, private communication, 2022.
\bibitem{SAID:DB}
    W.~J.~Briscoe, I.~I.~Strakovsky, and R.~L.~Workman, GWU CNS DAC SAID database located at http://gwdac.phys.gwu.edu/analysis/pr$_{-}$analysis.html .   
\bibitem{CLAS:DB}
    CLAS Physics Database is available through the JLab CLAS website:
    http://clasweb.jlab.org/physicsdb.
\bibitem{Data-DOI}
    The data supporting this research is openly available from the University of York Pure repository with DOI: 10.15124/99b659e3-e612-45f1-83f9-9122c9aa711c.
%--------------------------------------------------------------------
%\bibitem{Kim:2022ldz}
%    C.~Kim,
%    ``Measurement of the Helicity $\mathbb{E}$ for the $\gamma p \to \pi^0p$ Reaction in the Resonance Region,''
%    Ph.~D. dissertation, 
%    The George Washington University (2021);
%\bibitem{Iwamoto:2011dya}
%    H.~Iwamoto,
%    ``Helicity asymmetry measurement for $\pi^0$ photoproduction with FROST,''
%    Ph.~D. dissertation, 
%    The George Washington University (2011).
%\bibitem{Iwamoto:2012zza}
%    H.~Iwamoto [for CLAS Collaboration],
%    ``Helicity asymmetry $\mathbb{E}$ measurement for single $\pi^0$ photoproduction with a frozen spin target,'' in Proceedings of the 8th International Workshop on the Physics of Excited Nucleons: NSTAR2011, edited by V.~Burkert, M.~Jones, M.~Pennington, and D.~Richard, AIP\ Conf.\ Proc.\ \textbf{1432}, 275 (2012).
%\bibitem{Schott:2015fbn}
%    D.~Schott, W.~J.~Briscoe, and I.~Strakovsky [for CLAS Collaboration],
%    ``Helicity asymmetry measurement for \ensuremath{\pi}$^0$ photoproduction on the CLAS frozen spin target,'' in Proceedings of the 14th International Conference on Hadron Spectroscopy: Hadron2015, edited by M.~Pennington, AIP\ Conf.\ Proc.\ \textbf{1735}, 030016 (2016).
%\bibitem{Arndt:2006bf}
%    R.~A.~Arndt, W.~J.~Briscoe, I.~I.~Strakovsky, and R.~L.~Workman,
%    ``Extended partial-wave analysis of $\pi N$ scattering data,''
%    Phys.\ Rev.\ C\ \textbf{74}, 045205 (2006).
\end{thebibliography}
